Asymmetric Random Projections

Random projections (RP) are a popular tool for reducing dimensionality while preserving local geometry. In many applications the data set to be projected is given to us in advance, yet the current RP techniques do not make use of information about the data. In this paper, we provide a computationally light way to extract statistics from the data that allows designing a data dependent RP with superior performance compared to data-oblivious RP. We tackle scenarios such as matrix multiplication and linear regression/classification in which we wish to estimate inner products between pairs of vectors from two possibly different sources. Our technique takes advantage of the difference between the sources and is provably superior to oblivious RPs. Additionally, we provide extensive experiments comparing RPs with our approach showing significant performance lifts in fast matrix multiplication, regression and classification problems.

==> Data-Dependent Random Projections/suplementary.tex <==
\appendix


\section{Proofs of Section~\ref{sec:ddrp}} \label{sec:proof_ddrp}

\begin{proof} [Proof of Lemma~\ref{lem:iid_rp}]
We first observe that the estimate is indeed unbiased
\begin{align*}
    \E[\ip{Rx, Rw}] &= \E[x^\top R^\top Rw] \\
    &= x^\top\E[R^\top R]w \\
    &= x^\top w \\
    &= \ip{x,w}
\end{align*}
We move on to compute its variance. To that end, we begin with the case of $k=1$ where the dimension reduction is with a $d$ dimensional vector $r$ and denote by $r_i$ its $i$'th element. We compute the second moment explicitly; to that end we denote by $s_{2,2} = \E_{r_i,r_j} r_i^2 r_j^2$, $s_{4} = \E_{r_i } r_i^4$. For our distribution we have $s_{2,2}=1, s_{4} \leq 3$.
\begin{align*}
    \E_{r } \ip{x, r}^2 \ip{w, r}^2 &= \E_r \left( \sum_i x_i r_i \right)^2 \left( \sum_i w_i r_i \right)^2\\
 &= \E_{r} \left(\sum_i x_i r_i\right)^2 \left(\sum_i w_i r_i\right)^2 \\
&=\E_r \left(\sum_i x_i^2 r_i^2 +  \sum_{i \neq j} x_i x_j r_i r_j \right) \left(\sum_i w_i^2 r_i^2 + 2 \sum_{i < j} w_i w_j r_i r_j \right)\\
&= \E_r \left(\sum_i x_i^2 w_i^2 r_i^4 + 2 \sum_{i \neq j} x_i x_j w_i w_j r_i^2 r_j^2 + \sum_{i \neq j} x_i^2 w_j^2 r_i^2 r_j^2\right) \\
&= s_4 \sum_i x_i^2 w_i^2  + 2 s_{2,2} \sum_{i \neq j} x_i x_j w_i w_j  + s_{2,2} \sum_{i \neq j} x_i^2 w_j^2 \\
&= s_4 \sum_i x_i^2 w_i^2  + 2 s_{2,2}\left(\ip{x,w}^2 - \sum_i x_i^2 w_i^2\right) + s_{2,2} \sum_{i \neq j} x_i^2 w_j^2 \\
&= s_4 \sum_i x_i^2 w_i^2  + 2 s_{2,2}\left(\ip{x,w}^2 - \sum_i x_i^2 w_i^2\right) + s_{2,2} \left( \|x\|^2\|w\|^2 - \sum_i x_i^2 w_i^2 \right)  \\
&= \left(s_4 - 3s_{2,2}\right)  \sum_i x_i^2 w_i^2 + 2s_{2,2} \ip{x, w}^2 + s_{2,2} \|x\|^2 \|w\|^2 \\
&\leq 2\ip{x, w}^2 + \|x\|^2 \|w\|^2 \\
\end{align*}
We get that the variance of the estimate of $\ip{x,w}$ is
$$\Var \leq \ip{x,w}^2 + \|x\|\|w\|^2$$
For the case of $R$ being a matrix with target dimension $k$, since everything is i.i.d, the estimate is simply an average of $k$ independent estimates of target dimension 1, and the variance is the same as above, divided by $k$.
\end{proof}



\begin{proof} [Proof of Theorem~\ref{thm:full}]
Let $Q_X^\top Q_X = \Sigma_X, Q_W^\top Q_W = \Sigma_W$. Using the independence of $x$ and $w$ we get
\begin{align*}
& \E_{x,w}\|Ax\|^2\|(A^{\top})^{-1}w\|^2 \\ 
&= \Tr{A^{\top} A \Sigma_X}\Tr{(A^{-1} (A^{-1})^{\top}\Sigma_W}\\
&= \Tr{Q_X A^{\top} A Q_X^\top}\Tr{(Q_W A^{-1} (A^{-1})^{\top}Q_W^\top}&\\
&= \|A Q_X^\top\|^2_F \|A^{-\top} Q_W^\top\|^2_F&
\end{align*}
By Cauchy-Schwarz on the Frobenius Inner Product we get the universal lower bound:
\begin{align*}
     \Tr{ Q_X Q_W^{\top} } &= \langle A Q_X^\top, A^{-\top} Q_W^\top \rangle_F^2\\
&\leq \|A Q_X^\top\|^2_F \|A^{-\top} Q_W^\top\|^2_F 
\end{align*}
We use the Frobenius Inner Product
$\ip{X,Y}_F = \Tr{X^\top Y}$ and the Cauchy-Schwartz inequality stating that $\ip{X,Y}_F \leq \|X\|_F \|Y\|_F$. It implies that
\begin{align*}
\Tr{ Q_X Q_W^\top }^2 &= \Tr{ Q_X A^\top A^{-\top} Q_W^\top }^2\\
&= \ip{ A Q_X^\top, A^{-\top} Q_W^\top }_F^2 \\
&\leq \|A Q_X^\top\|^2_F \|A^{-\top} Q_W^\top\|^2_F \\
&= \E_{x,w}\|Ax\|^2\|A^{-\top}w\|^2 \end{align*}

Notice that this inequality happens for any factorization matrices $Q_X,Q_W$ and any invertible matrix $A$. Furthermore, the lefthand size is independent of $A$ and the righthand side is independent of $Q_X,Q_W$. It follows that if we find a specific triplet $Q_X,Q_W,A$ such that
\[ 
\ip{ A Q_X^\top, A^{-\top} Q_W^\top }_F^2 = \|A Q_X^\top\|^2_F \|A^{-\top} Q_W^\top\|^2_F
\]
we get that $Q_X,Q_W$ maximize the left expression and $A$ minimizes the right expression. Now, for two matrices $X,Y$ it holds that $\ip{X,Y}_F =  \|X\|_F \|Y\|_F$ only if $X=\lambda Y$ for some scalar $\lambda$. It follows that w.l.o.g.\ our matrix $A$ is such that 
$$ A Q_X^\top = A^{-\top} Q_W^\top$$
or conversely
$$ A^{\top}A Q_X^\top = Q_W^\top $$
Such a matrix $A$ can be found via CCA
\begin{lemma}[CCA]
Given two positive definite matrices $\Sigma_X, \Sigma_W$, we can pick matrix $A$ such that 
\[A  \Sigma_X A^\top =  A^{-\top} \Sigma_W A^{-1}  \]
If we decompose $\Sigma_X = Q_X^\top Q_X$, $\Sigma_W = Q_W^\top Q_W$, $Q_X Q_W^\top = U_{XW} D_{XW} V_{XW}^\top$, then we can set
\[ A = D_{XW}^{1/2} U_{XW}^\top Q_X^{-\top} \]
\[ A^{-\top} = D_{XW}^{1/2}V_{XW}^\top Q_W^{-\top} \]
Furthermore this choice of $A$ is independent of the decomposition of $\Sigma_X$ or $\Sigma_W$
\end{lemma}

We choose $Q_X$ arbitrarily and set $Q_W$ in a way that $Q_XQ_W^\top$ is symmetric and positive definite. This can be done by choosing an arbitrary $\hat{Q}_W$, decomposing $Q_X\hat{Q}_W^\top = \hat{U}\hat{D}\hat{V}^\top $ and setting $Q_W = \hat{U} \hat{V}^\top \hat{Q}_W$. Since $\hat{V},\hat{U}$ are orthogonal matrices we still have $Q_W^\top Q_W = \Sigma_W$. We also get that
$$ Q_XQ_W^\top = Q_X\hat{Q}_W^\top \hat{V}\hat{U}^\top =  \hat{U}\hat{D}\hat{V}^\top \hat{V} \hat{U}^\top = \hat{U}\hat{D}\hat{U}^\top$$

\noindent Using the terms above we can plug in the equation for $A^*$, the optimizer of the CCA problem, and obtain
\begin{align*}(A^*)^\top A^* Q_X^\top &= Q_W^\top V_{XW}^{-\top} D_{XW}^{-1/2} D_{XW}^{1/2} U_{XW}^\top  Q_X^{-\top} Q_X^\top\\ & = Q_W^\top V_{XW}^{-\top} U_{XW}^\top  \\
\end{align*}
Since we chose $Q_X,Q_W$ in a way that $Q_XQ_W^\top$ is psd we get that $V_{XW}=U_{XW}=\hat{U}$ and 
$$(A^*)^\top A^* Q_X^\top =Q_W^\top $$
as required.

Now that we obtained the minimizer $A^*$ we can compute the value of the expression.  $\Tr{Q_XQ_W^\top}$ equals the sum of the eigenvalues of the matrix which are the same as its singular values since it is psd. That is, the value of $\Phi(A^*)$ is the sum of the elements of $D_{XW}$. Notice that these elements do not depend on our choice of $Q_X,Q_W$ as that choice only affects the rotations $V_{XW}, U_{XW}$. With that in mind we can compute the values of $D_{XW}$ by considering the decomposition $Q_X =  D_X^{1/2} U_X^\top$, $Q_W =  D_W^{1/2} U_W^\top$, where $\Sigma_X = U_X D_X U_X^\top, \ \ \Sigma_W = U_W D_W U_W^\top$ are the singular value decompositions of $\Sigma_X,\Sigma_W$, we get that these values are exactly those obtained by multiplying the square roots of the eigenvalues of $\Sigma_X, \Sigma_W$ as required.


\end{proof}

\begin{proof} [Proof of Theorem~\ref{thm:fast}]
In what follows we use the fact that the Frobenius inner product of $M$ with a diagonal matrix only depends on the diagonal entries of $M$. That is, if $X$ is diagonal then for any matrix $M$ we have $\Tr{XM}=\Tr{X\diag{M}}$ where $\diag{M}$ is the matrix that is equal to $M$ on the diagonal and zero elsewhere. Using the fact the $A$ is diagonal we get
\begin{align*}
& \|A Q_X^\top \|_F^2 \|A^{-\top} Q_W^\top \|_F^2\\
&= \Tr{A^\top A \Sigma_X} \Tr{A^{-1} A^{-\top} \Sigma_W} \\ 
&= \Tr{A^\top A \diag{\Sigma_X}} \Tr{A^{-1} A^{-\top} \diag{\Sigma_W}}  
\end{align*}
This simple calculation shows us that restricting to diagonal pre-processing is equivalent to throwing away all of the off-diagonal information in our covariance matrices, and proceeding with the results of Theorem~\ref{thm:full}. The claim trivialy follows.

\end{proof}

% \newpage
% \section{Large Figures}
% \setlength{\textfloatsep}{5pt}
% \setlength{\intextsep}{5pt}
% \begin{figure}[h]

% \centering

% \begin{center}
%     Larger version of Figure \ref{fig:fmm_synthetic}
% \end{center}
% \begin{tabular}{cc}
%   \includegraphics[width=.32\linewidth]{"experiments/fmm/diag_diag_100_1000_100_distortion".png} & 
%   \includegraphics[width=.32\linewidth]{"experiments/fmm/rand_diag_100_1000_100_distortion".png} \\
%   \includegraphics[width=.32\linewidth]{"experiments/fmm/rand_randskew_100_1000_100_distortion".png}&
%   \includegraphics[width=.32\linewidth]{"experiments/fmm/rand_rand_100_1000_100_distortion".png}\\
%   \end{tabular}  
% %   \caption{Larger Figure \ref{fig:fmm_synthetic}}
% \end{figure}

% \begin{center}
%     Larger version of Figure \ref{fig:fmm_biological}
% \end{center}
% \begin{figure}[h]
% \centering
% \begin{tabular}{cc}
%   \includegraphics[width=.32\linewidth]{"experiments/fmm/arcene_5000_700_100_distortion".png} &
%   \includegraphics[width=.32\linewidth]{"experiments/fmm/arcene_700_5000_100_distortion".png} \\
%   \includegraphics[width=.32\linewidth]{"experiments/fmm/isolet_308_1559_100_distortion".png}&
%   \includegraphics[width=.32\linewidth]{"experiments/fmm/isolet_t_1559_308_100_distortion".png}\\
%   \end{tabular}
% %   \caption{ Larger Figure \ref{fig:fmm_biological}}
% \end{figure}

% \newpage
% \begin{center}
%     Larger version of Figure \ref{fig:fmm_sparse}
% \end{center}
% \begin{figure}[h]
% \centering
% \begin{tabular}{cc}
%   \includegraphics[width=.4\linewidth]{"experiments/fmm/go_sf_3853_2593_100_distortion".png} &
%   \includegraphics[width=.4\linewidth]{"experiments/fmm/go_sf_t_2593_3853_100_distortion".png} \\
%   \includegraphics[width=.4\linewidth]{"experiments/fmm/tw_oc_5673_5000_100_distortion".png}&
%   \includegraphics[width=.4\linewidth]{"experiments/fmm/tw_oc_t_5000_5673_100_distortion".png}\\
%   \end{tabular} 
% \end{figure}


% \begin{center}
%     Larger version of Figure \ref{fig:reg_linear}
% \end{center}
% \begin{figure}[h]
% \centering
% \begin{tabular}{cc}
%   \includegraphics[width=.4\linewidth]{"experiments/regression/slice_localization_384_53500_5_lamb_5_0".png} &
%   \includegraphics[width=.4\linewidth]{"experiments/regression/e2006_full_150360_16087_20_lamb_50_6".png} 
% %   \includegraphics[width4.3\linewidth]{"experiments/regression/e2006_full_150360_16087_20_lamb_50_5".png} \\
%   \end{tabular}
% %   Plotted empirical mean linear loss against hyper-parameter lambda. Slice localization dataset has 53500 samples with 384 features gathered from biological sources. We see the best results with $\lambda \sim -.50$. E2006 dataset is sparse data derived from term frequency–inverse document frequency (16087 samples, 150630 dimensional). Very little improvement for positive $\lambda$ and large blow up for negative values of $\lambda$. The isotropic prior causes huge blow up for the sparse data, but seems near optimal for the biological data.
% \end{figure}

% \newpage
% \begin{center}
%     Larger version of Figure \ref{fig:reg_logistic}
% \end{center}

% \begin{figure}[h]
% \centering
% \begin{tabular}{cc}
%   \includegraphics[width=.4\linewidth]{"experiments/regression/cifar_logistic_3072_1979_100_lamb_50_0".png} &
% =  \includegraphics[width=.4\linewidth]{"experiments/regression/rcv1_47236_20242_15_lamb_50_0".png}  \\
%   \end{tabular}
  
% %   plotted sklearn score (accuracy) against target dimension. Cifar dataset is image classification, 1979 samples with 3072 attributes projected 100 times. The accuracy is maximized around $\lambda \sim -.25$. RCV1 dataset is 20242 data points with 47236 feature and has accuracy maximized around $\lambda \sim .25$. In both cases the isotropic prior behaves well. 
% \end{figure}


\section{Additional Experiments} \label{app:more experiments}

\subsection{FMM synthetic data}\label{sec:synth}

For synthetic matrices we define a few distributions over matrices. In the first, called {\bf diag}, we first sample a $d$ dimensional vector of i.i.d Laplace variables. This determines a diagonal $d \times d$ covariance matrix. Now we sample $n$ i.i.d.\ rows to construct the matrix. The second distribution, called {\bf uniform}, we sample $d$ i.i.d.\ uniform variables in $[0,1]$ as the eigenvalues of the covariance and a random rotation for the eigenvectors. With the covariance matrix ready we sample $n$ i.i.d.\ rows. The third type called {\bf unifskew} is obtained by averaging two independent matrices one drawn from {\bf diag} and one from {\bf uniform}.
The pairs of synthetic matrices we consider are {\bf diag-diag}, {\bf uniform-diag}, {\bf uniform-unifskew}, {\bf uniform-uniform}. Every pair of matrices $X,W$ consists of two independently drawn matrices from the mentioned distribution.

For each of the $X,W$ pairs we compute the exact product $XW^\top$, and 3 approximate matrix products $(XR)(WR)^\top$ corresponding to three random projections $R$. The first, {\bf oblivious} is an oblivious random projection with i.i.d.\ signs. The second {\bf quick}, contains a pre-processing component based only on the diagonal entries of the covariance of $X$ and $W$.   The third, {\bf optimal}, contains the optimal pre-processing component based on CCA. 
For each approximate matrix product we compute the Squared Error, namely $\|XW^\top - (XR)(WR)^\top\|_F^2$ for multiple values of target dimension. We repeated the experiment 100 times to account for the noise coming from the randomness of $R$. 


For each of the three distributions detailed above, \textbf{diag}, \textbf{uniform}, \textbf{unifskew}, we draw 1000 samples from $\mathbb{R}^{100}$. We then form a matrices using these as columns, and look at the squared error over 100 random projections. The first experiment we conduct is looking at the mean squared error for two matrices, both with columns drawn from the \textbf{diag} distribution. For this experiment quick and optimal are equivalent (since the covariance matrix is diagonal) and nets around a 3x decrease in MSE, regardless of the target dimension. When comparing \textbf{diag} against \textbf{unif}, we use the same methodology. Here we see quick yields approximately a 1.5x decrease in MSE over oblivious, and optimal yields another 1.5x decrease in MSE from quick. When comparing \textbf{unif} against \textbf{unifskew} we get the same decreases as the previous experiement across all target dimensions. Finally we compare \textbf{unif} against \textbf{unif}. Here the quick projections yield the same MSE as oblivious projections, while optimal projections yield a 2x decrease in MSE.

These results demonstrate what we expect: when drawing from distributions whose covariance are mostly concentrated on the diagonal, quick random projections perform almost as well as optimal while requiring significantly less preprocessing time. In figure \ref{fig:fmm_synthetic} we plot the results of these experiments by plotting the mean squared error against different target dimensions. For each plot we also include dashed lines to show the standard deviation among the 100 random projections.




\begin{figure}[ht]
\begin{tabular}{cc}
  \includegraphics[width=.4\linewidth]{"experiments/fmm/diag_diag_100_1000_100_distortion".png} & 
  \includegraphics[width=.4\linewidth]{"experiments/fmm/rand_diag_100_1000_100_distortion".png} \\
  \includegraphics[width=.4\linewidth]{"experiments/fmm/rand_randskew_100_1000_100_distortion".png}&
  \includegraphics[width=.4\linewidth]{"experiments/fmm/rand_rand_100_1000_100_distortion".png}\\
  \end{tabular}  \caption{Synthetic Data FMM. Detailed in \S \ref{sec:synth}. Top left compares \textbf{diag} to \textbf{diag}. Top right compares \textbf{unif} to \textbf{diag}. Bottom left compares \textbf{unif} to \textbf{unifskew}. Bottom right compares \textbf{unif} to \textbf{unif}.}
  \label{fig:fmm_synthetic}
\end{figure}

